Simultaneous tiling

We discuss problems of simultaneous tiling. This means that we have an object (set, function) which tiles space with two or more different sets of translations. The most famous problem of this type is the Steinhaus problem which asks for a set simultaneously tiling the plane with all rotates of the integer lattice as translation sets.

==> gatz-1.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0}%
}%
\special{pdf:literal q}%
\begin{picture}( 342.938696, 167.111103)%
\special{pdf:literal \ASYraw{
 -317.824877 0.000000 m
 -151.338100 0.000000 l
 -151.338100 166.486778 l
 -317.824877 166.486778 l
 -317.824877 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-231.861169,83.555551)(0.000000,-0.469390){0}%
\end{picture}%
\kern -342.938696pt%
\special{pdf:literal Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-335.727831,83.555551)(-0.500000,-0.500000){$\Lambda$:}%
\special{pdf:literal q}%
\begin{picture}( 342.938696, 167.111103)%
\special{pdf:literal \ASYraw{
 -126.365083 0.000000 m
 40.121694 0.000000 l
 40.121694 166.486778 l
 -126.365083 166.486778 l
 -126.365083 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-39.683401,83.555551)(0.000000,-0.469390){0}%
\end{picture}%
\kern -342.938696pt%
\special{pdf:literal Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-101.772287,83.555551)(-0.500000,-0.500000){$\Lambda^*$:}%


==> gatz/gatz-1.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0}%
}%
\special{pdf:literal q}%
\begin{picture}( 342.938696, 167.111103)%
\special{pdf:literal \ASYraw{
 -317.824877 0.000000 m
 -151.338100 0.000000 l
 -151.338100 166.486778 l
 -317.824877 166.486778 l
 -317.824877 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-231.861169,83.555551)(0.000000,-0.469390){0}%
\end{picture}%
\kern -342.938696pt%
\special{pdf:literal Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-335.727831,83.555551)(-0.500000,-0.500000){$\Lambda$:}%
\special{pdf:literal q}%
\begin{picture}( 342.938696, 167.111103)%
\special{pdf:literal \ASYraw{
 -126.365083 0.000000 m
 40.121694 0.000000 l
 40.121694 166.486778 l
 -126.365083 166.486778 l
 -126.365083 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-39.683401,83.555551)(0.000000,-0.469390){0}%
\end{picture}%
\kern -342.938696pt%
\special{pdf:literal Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-101.772287,83.555551)(-0.500000,-0.500000){$\Lambda^*$:}%

